Relational Graph Attention Networks

We investigate Relational Graph Attention Networks, a class of models that extends non-relational graph attention mechanisms to incorporate relational information, opening up these methods to a wider variety of problems. A thorough evaluation of these models is performed, and comparisons are made against established benchmarks. To provide a meaningful comparison, we retrain Relational Graph Convolutional Networks, the spectral counterpart of Relational Graph Attention Networks, and evaluate them under the same conditions. We find that Relational Graph Attention Networks perform worse than anticipated, although some configurations are marginally beneficial for modelling molecular properties. We provide insights as to why this may be, and suggest both modifications to evaluation strategies, as well as directions to investigate for future work.

==> diagrams/one-dimensional-equivalence-example.tex <==
\begin{figure}[ht]
\begin{center}
  \begin{tikzpicture}[x=2.6cm, y=1.0cm, >=Stealth]
  \node [neuron] at (0, 0) (A) {$1$};
  \node [neuron] at (1, 0) (B) {$0$};
  \node [neuron] at (2, 0) (C) {$1$};

  % Self connections for 2
  \draw [->] (A) to[out=360-60,in=180+60,looseness=5] (A);
  \draw [->] (B) to[out=360-60,in=180+60,looseness=5] (B);
  \draw [->] (C) to[out=360-60,in=180+60,looseness=5] (C);

  \draw [red, ->] (B) -- (A);
  \draw [red, ->] (C) -- (B);
\end{tikzpicture}
\end{center}
\caption{Directed graph whose convolution corresponds to the one-dimensional convolution of the signal
  $\bmx=[1\;0\;1]$ with the kernel $\bmw=[2\;7]$. Convolutions with the kernel
  element 2 (7) are shown with black (red) arrows.}
\label{fig:one-dimensional-graph-conv}
\end{figure}


==> preamble/acronyms/f.tex <==
\newacronym{fs}{FS}{FastSent}
\newacronym{ft}{FT}{Fourier Transform}

==> sections/body/related-work.tex <==
\section{Related Work}
\label{sec:related-work}

\subsection{Generalising convolutions}
\subsubsection{Spectral approaches}
Spectral approaches define the convolutional operator using the spectral
representation of a graph. Notably, \cite{Bruna} was the first to generalise
\glspl{cnn} to graphs based on the spectrum of the graph Laplacian. However, their
approach involves the costly operation of eigendecomposition, the filters in the
spectral domain are not guaranteed to be localised in the spatial domain, and
the number of free parameters per filter are $\mathcal{O}(n)$ in the size of the
input \citep{Bronstein}. \cite{Henaff} proposed a variant with smooth spectral
multipliers, which guarantee spatially-localised filters and are
$\mathcal{O}(1)$ in the size of the input. Subsequently, \cite{Defferrard2016}
used Chebyshev polynomials as a basis for the filters which does not require
eigendecomposition. Using this insight, \cite{Kipf2016} restricted filters to a
1-hop neighborhood for a fast and scalable propagation rule.
\cite{Schlichtkrull2018} extended this approach to relational graphs by
computing a weighted average of the hidden representations of each relationship
type.

\subsubsection{Spatial approaches}
Spatial approaches define the convolutional operator in the spatial domain, i.e. directly on the graph. There are two major difficulties with this approach: there is the lack of shift invariance, and there is no inherent coordinate system in graphs. \cite{Duvenaud} learns a weight matrix per node degree to solve these problems, but is prohibitively slow for large graphs.  A more scalable approach was proposed by \cite{Atwood2016}, who define a convolution operation using random walks by considering a power series of a transition matrix with a separate weight matrix learnt for each neighbourhood size and graph feature. \cite{Monti} proposed using a mixture of Gaussian kernels defined on pseudo-coordinate systems local to nodes as convolutional operators. Further, they show previous approaches are special cases of their approach \citep{Masci, Boscaini2016}. 

\subsubsection{Hybrid approaches}
Hybrid approaches combine spectral and non-spectral approaches.
\cite{Shuman2016} generalises the windowed Fourier transform; a classic
technique allowing for an explicit trade-off between spatial and spectral
localisation through the choice of a window function  are among those that
have also extended wavelets to non-Euclidean domains to achieve a similar
effect.

\subsection{Attention mechanisms in graphs} 
Attention mechanisms aid models to focus on relevant parts of the input.
\cite{Velickovic2017} proposes a shared attention mechanism where attention
coefficients between nodes depend on their respective features. A similar
architecture is given by \cite{Thekumparampil2018}, which uses a weighted cosine
similarity between node features instead of training an MLP to compute the
attention coefficients. Further, \cite{Shang2018} proposed attention
coefficients which solely depend on the edge types, but do not leverage (often
available) node features.

